Classifier Language Models: Unifying Sparse Finetuning and Adaptive Tokenization for Specialized Classification Tasks

Semantic text classification requires the understanding of the contextual significance of specific tokens rather than surface-level patterns or keywords (as in rule-based or statistical text classification), making large language models (LLMs) well-suited for this task. However, semantic classification applications in industry, like customer intent detection or semantic role labeling, tend to be highly specialized. They require annotation by domain experts in contrast to general-purpose corpora for pretraining. Further, they typically require high inference throughputs which limits the model size from latency and cost perspectives. Thus, for a range of specialized classification tasks, the preferred solution is to develop customized classifiers by finetuning smaller language models (e.g., mini-encoders, small language models). In this work, we develop a token-driven sparse finetuning strategy to adapt small language models to specialized classification tasks. We identify and finetune a small sensitive subset of model parameters by leveraging task-specific token constructs in the finetuning dataset, while leaving most of the pretrained weights unchanged. Unlike adapter approaches such as low rank adaptation (LoRA), we do not introduce additional parameters to the model. Our approach identifies highly relevant semantic tokens (case study in the Appendix) and outperforms end-to-end finetuning, LoRA, layer selection, and prefix tuning on five diverse semantic classification tasks. We achieve greater stability and half the training costs vs. end-to-end finetuning.

==> 02-RelatedWork.tex <==
\section{Related Work}
\label{related_work}
Personal identifiable information (PII) is a sensitive topic in real-world machine-learning applications due to legal, ethical, and regulatory restrictions. Data privacy and artifical/synthetic data creation are important topics in this context~\cite{sei2022privacy, qinl2022synthesizing}. There are numerous advantages to synthetic PII data; First, they can be shared without privacy constraints, and second, their volume and characteristics can be controlled to diversify data variations, and accurately evaluate large scale systems~\cite{christen2009accurate}. Previous work has introduced corruption, noise, and distributional changes to synthetic PII data ~\cite{christen2013flexible} to test the robustness of machine-learning solutions. 

In this work, we are particularly interested in evaluating deduplication for PII, broadly referred as Entity Resolution (ER) , the process of consolidating records that represent the same real-world entity \cite{getoor2012entity,KondaDCDABLPZNP16}. ER typically consists of two primary phases: blocking and matching. The blocking phase generates candidate pairs of entities, and the matching phase provides a final match/no-match decision for each candidate pair. Our benchmark provides two datasets, one to evaluate each of these two phases.

A considerable body of work has proposed deep-learning techniques for the matching phase \cite{DBLP:conf/acl/KasaiQGLP19,DBLP:conf/vldb/PeetersBG20,ditto2021,DBLP:conf/sigmod/Miao0021,akbarian2022probing,yao2022entity}. Recent work proposes contrastive learning methods and/or labeled data for BERT-based models in ER tasks~\cite{ditto2021,wang2022sudowoodo,peeters2022supervised}, as well as cutting edge large language models (LLMs) ~\cite{peeters2023using}. We evaluate a representative set of methods in our experiments (\cref{experiments}), and show that our dataset proves challenging even to state-of-the-art methods.

However, we note that the blocking phase is critical to reduce the computational load of the matching system, since the number of candidate pairs potentially grows as the square of the dataset size. More recently, ~\cite{papadakis2023benchmarking} and ~\cite{zeakis2023pre} have benchmarked blocking workflows. The challenge of the blocking phase is to achieve a minimal candidate set to reduce computation while maximizing the identification of true matches. To better evaluate blocking methods, we also provide a large blocking dataset of one million records. An ideal blocking method can correctly identify all matching pairs in our matching dataset, while reducing the overall candidate count. 

% have performed experimental studies on traditional blocking workflows and embedding-based nearest-neighbor search methods. They analyze the relative performance of the main representatives per category over numerous established datasets. 
%However, these works do not study the generalization capabilities of state-of-the-art methods in the literature, and they overlook the latest advancements in the Information Retrieval (IR) literature which is important because the entity blocking problem can also be solved using IR methods. %Our work focuses on the generalization capabilities of latest advancements in both the entity resolution and information retrieval literature. 

% Blocking is pivotal for large datasets, , making a naive approach computationally prohibitive, especially for intricate deep learning models \cite{wang2022sudowoodo,ditto2021}. The challenge of the blocking phase is to achieve a minimal candidate set to reduce computation while maximizing the identification of true matches.



% The research community has proposed a variety of blocking techniques, including rule-based blocking \cite{DBLP:conf/sigmod/DasCDNKDARP17,GokhaleDDNRSZ14,paulsen2023sparkly}, schema-agnostic blocking \cite{DBLP:journals/tkde/SimoniniPPB19}, meta-blocking \cite{DBLP:journals/pvldb/SimoniniBJ16}, deep learning techniques \cite{DBLP:journals/pvldb/ThirumuruganathanLTOGPFD21,DBLP:conf/wsdm/ZhangWSDFP20}, and Locality-Sensitive Hashing (LSH)-based blocking techniques \cite{borthwick2020scalable}. 
% %These methods can manage billions of items for entity matching. Most recently, Sparkly~\cite{paulsen2023sparkly} is a TF-IDF based method and achieves state-of-the-art performance on various datasets. 

%  These models are refined u to generate item-embeddings. Similar item pairs can then be discerned by executing a similarity search on the embeddings. For instance, Peeters et al. \cite{peeters2022supervised} proposed R-SupCon, a supervised contrastive learning model for product matching, utilizing the learned embeddings for blocking. %However, as R-SupCon's learning objective is oriented towards matching - essentially a binary classification task - the embeddings may not accurately capture the similarity of data items necessary for effective blocking.

% Entity blocking can also be framed as an Information Retrieval (IR) task. Recent literature in IR \cite{tonellotto2022lecture} has seen methods such as DPR \cite{karpukhin2020dpr}, GTR \cite{ni2021GRT}, and Contriever \cite{izacard2021contriever}, which utilize Pre-trained Language Model-based (PLM) methods to learn dense document representations. Candidate pairs can be identified by conducting a similarity search on these dense representations using FAISS \cite{johnson2019faiss}. %Conversely, Splade++ \cite{splade++} learns sparse representations and constructs an inverted index for lexical matching. %This fundamentally circumvents the necessity for pair-wise comparison and scales appropriately to large datasets. The out-of-distribution generalization capabilities has been studied in the IR literature~\cite{thakur2021beir}, and the evaluations incidate neural retrievers or rankers can poorly generalize to different domains/datasets.

==> 03-Methodology.tex <==
\section{BPID Dataset Construction}
\label{methodology}

In this section, we describe our generation approach for our benchmark dataset. We include five personally identifiable attributes - the name, any physical addresses, email addresses, phone numbers associated with the individual, and their date of birth, to match or not-match a pair of personal profiles. We first collect raw values for each of the five attributes from the below sources:

\begin{itemize}
\item \textbf{Name} : We generated artificial names by combining first names from the SSA popular baby names dataset\footnote{https://www.ssa.gov/oact/babynames/} and the Census Bureau popular surnames dataset\footnote{https://www.census.gov/topics/population/genealogy/data.html}.
\item \textbf{Physical Addresses} : We randomly choose physical addresses located in the United States from the USDOT National Address Database\footnote{https://www.transportation.gov/gis/national-address-database}.
\item \textbf{Email Addresses} : We generate realistic email addresses by combining parts of the names with additional keywords or numerical strings, and a randomly chosen domain name.
\item \textbf{Phone Numbers} : We combine country or area codes with randomly generated phone number values.
\item \textbf{Date-of-Birth} : We select random dates-of-birth ranging from 1900 to 2024.
\end{itemize}

Further, we randomly set ~20\% of the attribute values to empty strings to introduce missing entries~\cite{sei2022privacy}.

\subsection{Synthetic Profile Construction}
\label{blocking_dataset}
We generate synthetic individual profiles by combining randomly chosen values of the name, physical addresses, phone numbers, date-of-birth, and email addresses that exhibit similarities to the chosen name. We provide a synthetic sample profile constructed in this manner below:
\begin{verbatim}
SYNTHETIC PERSONAL PROFILE
    "fullname": "harold stickelman",
    "phonenumbers": ["9516784827", "9095194618"],
    "emailaddresses": ["stickelman2@verizon.net"],
    "addresses": ["40489 VIA CAMPOSE COMURRIETA CA 92562"],
    "birthdate": "1990-11-14"
\end{verbatim}  
We then select and manually generate modified versions of ten thousand of these profiles to construct the matching dataset, and ask human annotators to judge whether these ten thousand original and modified profile pairs represent the same individual, or two different identities. We detail the modification and annotation process for the matching dataset in the following subsections.

\subsection{Profile Modification by Trained Human Annotators}
\label{human-aug}
Consider the following synthetic profile, which we provide to our human annotators,
\begin{verbatim}
ORIGINAL PERSONAL PROFILE PROVIDED TO ANNOTATORS
    "fullname": "harold stickelman",
    "phonenumbers": ["9516784827", "9095194618"],
    "emailaddresses": ["stickelman2@verizon.net"],
    "addresses": ["40489 VIA CAMPOSE COMURRIETA CA 92562"],
    "birthdate": "1990-11-14"
\end{verbatim}  

We instruct our annotators to introduce variations in one or more attribute values in the above personal profile. Annotators are permitted to modify values, insert new values, or delete existing values of each of the five attributes, while maintaining similarities to the original profile to optimize sample difficulty. Some sample variations generated by our annotators are as follows:

\begin{verbatim}
POSITIVE MODIFIED PROFILE GENERATED BY ANNOTATORS 
(UNANIMOUS MATCH TO ORIGINAL)
    "fullname": "h stickel man",
    "phonenumbers": [],
    "emailaddresses": ["stickelman2@verizon.net"],
    "addresses": [],
    "birthdate": "1990 Nov"

NEGATIVE MODIFIED PROFILE GENERATED BY ANNOTATORS 
(UNANIMOUS NOT A MATCH TO ORIGINAL)
    "fullname": "harriet m stickelman",
    "phonenumbers": ["9516784827", "9095194618"],
    "emailaddresses": ["stickelman2@verizon.net"],
    "addresses": ["40489 VIA CAMPOSE COMURRIETA CA 92562"],
    "birthdate": "1993 Jun 19"
\end{verbatim}
The above process enables us to generate challenging pairs of matching and non-matching personal profile pairs to test the accuracy of an identity deduplication system.

\subsection{Automated Profile Modifications}
\label{heuristic-aug}
This section describes the programmatic modification and variations of raw attribute values introduced by us in the benchmark dataset, in addition to the human generated modifications.

\subsubsection{Positive Name Variantions}
A name variant is an alternative of a name that is considered to be equivalent to that name but which differs from the name in its particular external form. In other words, the two names are considered somehow equivalent and can be substituted for the other in most cases. Name variants occur for many reasons including spelling variations (e.g., Geoff and Jeff), nicknames (e.g., Bill for William), abbreviations (e.g., GPE for Guadalupe), cognates or translations (e.g., Peter for Pierre), cultural differences (e.g., Michael in English vs Michel in French), abbreviations and ordering (e.g., JPR Shields from Roberts Pierre John Shields) and common typographical errors (e.g., Chad vs. Cjad).


\subsubsection{Negative Name Variants}
This includes names that look similar at first glance but are likely to refer to different individuals. For instance, "Jon" is often a short form of "Jonathan" while "John" is a standalone name. Despite their similar appearance and pronunciation, they are distinct. Similarly, "Marc" and "Mark" are both given names typically pronounced the same way, potentially referring to different people. Gender variations are male-female name pairs that share a letters or phonetic sounds, making them appear similar, while clearly referring to individuals of different genders. For instance, Daniel (male) and Danielle (female) share a base ("Dan"), Jon (male) and Jen (female) are typographically similar, and Paula (female) is the feminine form of Paul (male).
        % \begin{itemize}
        %     \item Daniel and Danielle: These names share a base ("Dan") with "Danielle" typically being the feminine form of "Daniel."
        %     \item Jon and Jen: These names and typographically similar, despite "Jon" typically denoting a male name and "Jen" a female name.
        %     % \item Michael and Michaela: "Michaela" is the feminine form of "Michael"
        %     \item Paul and Paula: "Paula" is the feminine form of "Paul"
        %     % \item Alex and Alexa/Alexis: "Alex" can be short for Alexander or Alexandra while "Alexa" and "Alexis" are more commonly used for females.
        %     % \item Victor and Victoria: "Victoria" is the feminine form of "Victor"
        % \end{itemi

\subsubsection{Variant Generation}
To generate positive and negative name variations, we select similar candidate pairs of first names (e.g., \textit{Mary} vs \textit{Mark}) from our raw name values, and ask three annotators to judge each pair as a match, no-match, or ambiguous. We then include name pairs where all annotators agree to a match or no-match decision in our benchmark dataset. Note that matching pairs that include a positive name pairing (e.g., \text{Larry} vs. \text{Lawrence}) can be matched by the annotators depending on the other attribute values, while those with a negative pairing (e.g., \textit{Mary} vs. \textit{Mark}) will not be matched since they denote different individuals).


% \subsubsection{Business Listings}
% Business listings sometimes appear under different names due to various reasons such as branding strategies, mergers and acquisitions, subsidiaries, or simply variations in the naming across different locations or services. Despite the differences in names, these listings might actually represent the same business entity or corporation.

% \begin{itemize}
%     \item Positive business variations
%         \begin{itemize}
%             \item Cabo esperanza llc vs. cabo villa del sol llc
%             \item pcs partners vs. pcs metro computing
%             \item dtw landstar vs. landstar system inc.
%             \item fred motors vs. fred automotive services
%             \item gil development inc vs gil sunset villas inc
%             \item astrox development exploration co llc vs. astrox corp of boerne inc.
%             \item palace interactive inc. vs palace network llc
%             \item engels family partnership gp llc vs. efp llc
%         \end{itemize}
%     \item Negative business variations
%         \begin{itemize}
%             \item Hiatt legal vs. hiatt terry welding co.
%             \item Courtyard by Marriott vs. Courtyard plumbing services inc.
%             \item Fred motors vs. Fred’s barbecue grill
%         \end{itemize}
% \end{itemize}

\subsubsection{Physical Address Variations}

Our benchmark encompasses format variations to the address, replacement or deletion of different parts of each attribute (e.g., zip code, street address, city, or state in the address attribute), introduction of contradicting information (e.g., 101 Lincoln Ave Chicago IL vs. 101 Lincoln Ave Seattle WA), and semantic variations such as one hundred and fourth vs. 104th (positive) or Lombard Ave vs. Lombard Avenue (positive) or Lincoln Street North vs. Lincoln Street South (negative).

\subsubsection{Date-of-Birth, Phone Number and Email Variations}
Our benchmark contains format variations and incomplete or partial dates. Analogously, we introduce variations to the phone numbers, and email address fields, where we drop or retain parts of the entry such that they still indicate the same underlying value.

\subsection{Match/No-Match Annotation Process}

 We perform the pairwise match/no-match annotation process as follows. We first choose a raw personal profile, and a modified version that is generated by combining the approaches described in \cref{human-aug} and \cref{heuristic-aug}. We then present both the original and the modified versions of the profile to three trained human annotators. Each annotator is asked to fill in the below details.
\begin{enumerate}
    \item Evaluate the extent of match between the attribute values in the original and modified profile.
        \begin{itemize}
            \item Name - match/neutral/no-match
            \item Email - match/neutral/no-match
            \item Phone - match/neutral/no-match
            \item Address - match/neutral/no-match
            \item DOB - match/neutral/no-match
        \end{itemize}
    \item Provide the overall assessment - match/neutral/no-match.
\end{enumerate}

We asked three different annotators to judge if each modified profile with the variations should be matched to the original profile, or be considered a different individual. We obtained an agreement rate of 83\%, and only included the pairs where all three annotators unanimously decided a match or a no-match overall assessment.

\subsection{Benchmark Dataset Statistics}

Our final benchmark consists of two datasets. Our blocking dataset contains one million synthetic profiles including both, the raw profiles constructed in Section 3.1 as well as the augmented profiles from Sections 3.2, 3.3. The blocking dataset has an missing rate of 17.6\% over all five attributes. Names and dates-of-birth are present in 85.5\%, 85\% of the profiles respectively. We observe the average number of phone numbers, addresses, and emails per profile to be 1.2, 1.2, and 1.3 respectively. 

Second, our matching dataset contains ten-thousand pairs of personal profiles from Sections 3.2, 3.3 marked as matches or no-matches as detailed in Section 3.4. We also include every profile in the matching dataset as part of the blocking dataset to evaluate blocking methods. A perfect blocking method should correctly identify every pair in our matching dataset from the blocking dataset (i.e., have a high recall), while a perfect matching method should correctly classify each pair in the matching dataset as a match or no-match (i.e., have a high accuracy). The matching dataset contains ten thousand pairs of profiles with an attribute missing rate of 18.2\%, names and dates-of-birth present in 84.9\%, 84.5\% of the profiles, and an average of 1.17, phone numbers, 1.2 addresses, and 1.33 emails per profile. Our annotators unanimously judged 3472/10000 pairs as matches, and 6528/10000 as no-match pairs.

==> 04-Experiments.tex <==
\section{Evaluations}
\label{experiments}

In this section, we provide results for both the blocking dataset (which contains one million unannotated profiles) and the matching dataset, which contains ten-thousand profile pairs with match/no-match human annotations. Note that the set of profiles in the matching set is a subset of the blocking set. We evaluate state-of-the-art entity matching and blocking methods over our benchmark datasets. Our matching methods include a traditional supervised \textbf{Random Forest}~\cite{primpeli2020profiling}, pre-trained language model based methods, \textbf{Ditto}~\cite{ditto2021} and \textbf{Sudowoodo}~\cite{wang2022sudowoodo}, and \textbf{LLM-based methods}~\cite{peeters2023chatem}. We designed a LLM prompt (provided in \cref{prompt}) to determine if two profiles represent the same individual, and applied the prompt to various cutting-edge LLMs including Anthropic model Claude3-Sonnet, Meta AI \textbf{Llama3-70B-instruct}~\cite{meta2024introducing}, Mistral AI \textbf{Mistral large}~\footnote{https://mistral.ai/news/mistral-large/}, and OpenAI \textbf{GPT4}~\cite{achiam2023gpt}. We use the F1 score on the annotated matching dataset as our evaluation metric.

We selected \textbf{Sudowoodo}~\cite{wang2022sudowoodo},  \textbf{NLSHBlock}~\cite{wang2024neurallsh}, \textbf{Sparkly}~\cite{paulsen2023sparkly}, and \textbf{Contriever}~\cite{izacard2021contriever} for the blocking task. We measure the recall (the percentage of the matched pairs in the matching dataset that be retrieved from the blocking dataset) and the candidate set size generated by each method. Note that a higher recall and lower candidate size are preferred for blocking methods. %These methods cover pre-trained language model based solutions, traditional TF-IDF based solution, and dense information retrieval solutions. %We set a target recall 0.95 for each method and report their candidate set size to achieve that recall. We note that the target recall is a realistic goal in real-world applications, but specific application may require different target recall after considering the trade-off between cost and accuracy. We run the methods over the blocking set and calculate the recall by counting the number of occurrence of matched pairs from the matching set.

\subsection{Entity Matching results}
Table~\ref{tab:entity_matching} shows the F1 scores of various methods on the matching set. The results indicate that our dataset proves challenging for methods from all categories - even the most capable LLMs cannot achieve a satisfactory F1 score with the following prompt on our benchmark dataset. 
\begin{table}[h]
\vspace{-1em}

\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
Method 1 & Type & Precision & Recall & F1 \\
\hline
Random Forest & Traditional &0.528&0.716&0.608\\
%SVM~\cite{primpeli2020profiling} & Traditional &&&\\
Ditto & PLM & 0.728 & \underline{0.686} & \underline{0.701} \\
Sudowoodo & PLM & 0.738 & 0.670 & \textbf{0.702} \\
%Claude3-Opus & LLM & \underline{0.75} & 0.68 & \underline{0.72} \\
Claude3-Sonnet & LLM & 0.576 & \textbf{0.756} & 0.653 \\
%Claude3-Haiku& LLM & 0.61 & 0.54 & 0.579 \\
%Llama3-8B-instruct& LLM & 0.46 & 0.44 & 0.448 \\
Llama3-70B-instruct& LLM & 0.691 & 0.610 &  0.648\\
%Mistral 7B& LLM & 0.58 & 0.61 & 0.593 \\
%Mistral 8x7B& LLM & 0.63 & 0.65 & 0.641 \\
Mistral large& LLM & \underline{0.762} & {0.407} & 0.530 \\
GPT-4-turbo& LLM & \textbf{0.764} & {0.525} & {0.622} \\
\hline
\end{tabular}
\caption{F1 scores on evaluated matching methods. Bold font indicates the best performance and the underline indicates runner-up.}
\vspace{-23pt}
\label{tab:entity_matching}
\end{table}

We use the following prompt to evaluate LLM performance.
\begin{flushleft}
\label{prompt}
\texttt{\textbf{Instruction } }
Task description: You are a profile annotator and you need to evaluate the similarity between two profiles with the following guideline. Each profile consists of 5 different attributes:
\textit{phone}, \textit{email}, \textit{fullname}, \textit{addresses}, \textit{birthdate}.\
You need to carefully compare each attribute and make the match / no-match decision on the given profile pair. \\
Keep the these principles in mind when making a decision.\\
\textbf{Principle 1}.  Allow slight string variations of "common sense"/"human error", including upper/lower case, swapped positions of words in a string, absence/errors of country code, simple typos, date format, string synonyms. However, if two names have different first names, consider them as different people.\\
\textbf{Principle 2}. One element match between lists is considered as a match for the attribute: three attributes contain(phonenumbers, emailaddresses, addresses) a list of values, meaning one person can have more than one phonenumber/email/address. If two profiles have any email/phone/address in common, that means a "match" in this attribute. For example:
    sim( [chris.paul@gmail.com, cp3@yahoo.com], [nba\_champ123@amazon.com, chris.paul@gmail.com]) = match. This is because both email lists have "chris.paul@gmail.com".\\
\textbf{Principle 3}. Ignore invalid attribute values or values without enough information.\\
\textbf{Principle 4}. Make the decision based on holistic evaluation over all valid attributes. Only match two profiles if there is sufficient evidence.\\
Here are two personal profiles, please strictly follow the above guideline and use the below template to answer whether they are the same person:\\

\quad Analysis: [reasons for final decision about whether these two profiles should be matched or not]\\
\quad Answer: [Yes or No]

    Here are the two profiles:
\iffalse
Task description: You are a profile annotator and you need to evaluate the similarity between two profiles with the following guideline.
Each profile consists of 5 different attributes:\\
\textit{phone}, \textit{email}, \textit{fullname}, \textit{addresses}, \textit{birthdate}.\\
You need to carefully compare each attribute and make the match/no-match decision on the given profile pair. Keep these principles in mind when making a decision.\\

Principle 1.  Allow string variations of "common sense"/"human error", including upper/lower case, arrangement of strings, absence/errors of country code, simple typos, date format, string synonyms.\\
Principle 2. One element match between lists is considered as a match for the attribute: three attributes contain(phonenumbers, emailaddresses, addresses) a list of values, meaning one person can have more than one phonenumber/email/address. If two profiles have any email/phone/address in common, that means a "match" in this attribute. For example:
    sim( [chris.paul@gmail.com, cp3@yahoo.com], [nba\_champ123@amazon.com, chris.paul@gmail.com]) = match
    Both email lists have "chris.paul@gmail.com". \\
Principle 3. Make the decision based on holistic evaluation over all attributes. Only match two profiles if there is strong evidence. \\
Here are two personal profiles, please strictly follow the above guideline to tell me whether they refer to the same person. Answer "Match" or "No-Match".
\fi 
[\textbf{Profile 1}], [\textbf{Profile 2}].\\ 
Analyze step by step in plain text.\\
\end{flushleft}


\vspace{-1em}

\subsection{Blocking results}
Table~\ref{tab:blocking} shows the blocking performance of the evaluated methods on three metrics, recall, candidate set size (CSS), and time used for retrieving the candidates. We note that none of the valuated methods achieves over 80\% recall at a reasonable CSS. %Note that recall is the percentage of the matched pairs in the generated candidate set, while CSS is the total number of generated candidates. 
\begin{table}[h]
\vspace{-0.5em}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
Method & Recall & CSS (M=$10^6$)& Blocking time\\
\hline
%DeepBlocker &0.95 & 10M&\\
Sudowoodo~\cite{wang2022sudowoodo} &\underline{0.743} & 10M&6min\\
NLSHBlock~\cite{wang2024neurallsh} &0.650 & 10M&13min\\
Sparkly~\cite{paulsen2023sparkly} &0.627 & {10M}& 4min\\
Contriever~\cite{izacard2021contriever} &\textbf{0.758} & {10M}& 33min\\
%Splade++ &0.95 & 5M&\\
\hline
\end{tabular}
\caption{Recalls, Candidate Set Sizes (CSS), and blocking runtimes for each method. }%Bold font indicates the best performance and the underline indicates runner-up.}
\vspace{-20pt}
\label{tab:blocking}
\vspace{-1em}

\end{table}


==> 05-Conclusion.tex <==
\section{Conclusion}
In this paper, we introduce the first fully public benchmark dataset to facilitate the evaluation of data deduplication methods for personally identifiable information (PII). Our dataset is meticulously designed to provide a rigorous and challenging testbed, surpassing the limitations of simplistic rules or heuristic techniques. Even state-of-the-art large language models (LLMs), such as OpenAI's GPT-4, exhibit non-trivial error rates on our dataset, underscoring the complexity of the task and setting a high bar for evaluation. Through this benchmark, we aim to foster advancements in PII data deduplication, promoting the development of innovative methods that prioritize privacy and data security while enabling effective data management and analysis.

==> sections/abstract.tex <==
\begin{abstract}
    % As large-scale language models become the standard for text generation, there is a greater need to tailor the generations to be more or less concise, targeted, and informative, depending on the audience/application. Existing control approaches primarily adjust the semantic (\eg emotion, topics), structural (\eg syntax tree, parts-of-speech), and lexical (\eg keyword/phrase inclusion) properties of text, but are insufficient to accomplish complex objectives such as pacing which control the complexity and readability of the text. In this paper, we introduce \textsc{Cev-LM} - a lightweight, semi-autoregressive language model that utilizes constrained edit vectors to control three complementary metrics (speed, volume, and circuitousness) that quantify the shape of text (\eg pacing of content). We study an extensive set of state-of-the-art CTG models and find that \textsc{Cev-LM} provides significantly more targeted and precise control of these three metrics while preserving semantic content, using less training data, and containing fewer parameters.\footnote{Our code and data are accessible at this link \url{https://github.com/CrowdDynamicsLab/CEVLM}}
    % By leveraging the powerful natural language understanding of pre-trained LMs like BERT while fine-tuning them on domain data, we can enable cutting-edge AI capabilities tailored to the unique language properties and challenges of specialized verticals. However, fine-training strategies are dependent on the input structure presented at finetuning time, and in turn, the input structure primarily depends on the tokenization strategy, tokenizer vocabulary, and token structure in the input samples. While large language models such as OpenAI GPT-4 can often get away with generic tokenizers owing to their compute capacity and massive training data volumes, specialized language models are typically smaller in size, and trained on much smaller human curated domain-specific dataset.
    
    % We identify a synergistic training strategy to leverage the limited domain-specific training data optimally - first, by developing a domain-specific tokenization strategy, and second, by efficiently finetuning a small subset of the model parameters to adapt to the specialized task(s). We show that adaptive tokenization enables and requires parameter-efficient finetuning to truly shine in a specialized domain. The resulting model provides higher performance and a greater ability to generalize than either of the two approaches in isolation.

    %  However, specialized s

    % Cutting edge large language models (LLMs) such as Anthropic Claude-3\footnote{https://www.anthropic.com/claude}, Mistral Large\footnote{https://mistral.ai/news/mistral-large/}, and their open-source counterparts dominate general-purpose language understanding benchmarks\footnote{https://paperswithcode.com/sota/multi-task-language-understanding-on-mmlu}. 


  % Semantic classification requires an understanding of the contextual significance of specific tokens rather than just surface-level patterns or keywords (as in rule-based or simple statistical classification), making large language models (LLMs) well-suited for this task. However, semantic classification tasks in industry applications (e.g., user intent detection, semantic role labeling) tend to be highly specialized. They require labeled data annotated by domain experts in contrast to general-purpose pretraining corpora. Further, they typically require very high inference throughputs which limits the model size from a latency and cost perspective. Thus, for a range of specialized classification tasks, the preferred solution is to develop customized classifiers by finetuning smaller language models (e.g., mini-encoders, small language models). 

    
    Semantic text classification requires the understanding of the contextual significance of specific tokens rather than surface-level patterns or keywords (as in rule-based or  statistical text classification), making large language models (LLMs) well-suited for this task. However, semantic classification applications in industry, like customer intent detection or semantic role labeling, tend to be highly specialized. They require annotation by domain experts in contrast to general-purpose corpora for pretraining. Further, they typically require high inference throughputs which limits the model size from latency and cost perspectives. Thus, for a range of specialized classification tasks, the preferred solution is to develop customized classifiers by finetuning smaller language models (e.g., mini-encoders, small language models). 

    In this work, we develop a token-driven sparse finetuning strategy to adapt small language models to specialized classification tasks. We identify and finetune a small sensitive subset of model parameters by leveraging task-specific token constructs in the finetuning dataset, while leaving most of the pretrained weights unchanged. Unlike adapter approaches such as low rank adaptation (LoRA), we do not introduce additional parameters to the model. Our approach identifies highly relevant semantic tokens (case study in \cref{appendix:tokens}) and outperforms end-to-end finetuning, LoRA, layer selection, and prefix tuning on five diverse semantic classification tasks. We achieve greater stability and half the training costs vs. end-to-end finetuning.




\end{abstract}

==> sections/ethics_statement.tex <==
\section*{Ethics Statement}
By nature of being trained on data from the internet and because large language models tend to memorize patterns without understanding the language or implications, our approach is susceptible to generating incorrect~\cite{zellers2019defending, maynez2020faithfulness, pagnoni2021understanding} or biased information as well as toxic language~\cite{wallace2019universal, gehman-etal-2020-realtoxicityprompts, sheng2021societal}. Although most studies have been conducted on autoregressive frameworks~\cite{bender2021dangers}, \textsc{Cev-LM} is still prone to such problems and future research is necessary to mitigate these issues. However, our framework attempts to achieve controllable outcomes, and future work can experiment with utilizing controllability to address the aforementioned challenges~\cite{liu-etal-2021-dexperts, han2022ssd}. Conversely, controllability can be utilized for malicious use cases, and we should ensure that future work continues to defend against such use cases by ensuring released data and models are protected against harmful/de-anonymized content. 

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


\begin{figure}[b]
\centering  \includegraphics[width=0.22\textwidth]{figs/intro-new2.pdf}
  \vspace{-20pt}
  \caption{Task-specific tokenization helps finetune sensitive model parameters, while reusing a majority of the pretraining weights.}
  \label{fig:intro1}
  \vspace{-49pt}
\end{figure}

Cutting edge large language models (LLMs) such as Anthropic Claude-3\footnote{https://www.anthropic.com/claude} and OpenAI GPT-4~\footnote{https://openai.com/index/gpt-4/} dominate general-purpose language understanding benchmarks\footnote{https://paperswithcode.com/sota/multi-task-language-understanding-on-mmlu}. Although these models show strong language understanding~\cite{mmlu}, they are not optimized for specialized semantic classification tasks requiring domain expertise~\cite{nips2024llm}; for example, semantic role labeling in news content\footnote{https://paperswithcode.com/sota/semantic-role-labeling-on-ontonotes} where the best results belong to smaller task-specific models. In addition, large-scale applications serve thousands of classification queries per second~\cite{scale1}, which is prohibitively expensive for large models. Thus, there is an increasing focus on developing specialized, cost-effective language models for large-scale semantic classification tasks.

\begin{figure*}[]
  \centering
\includegraphics[width=0.9\textwidth]{figs/intro-big-img.pdf}
  \caption{We provide an illustration of prior sparse finetuning approaches compared to our proposed approach. The highlighted parameters indicate the trainable components under each method.}
  \label{fig:intro2}
\end{figure*}
Within the specialized model arena, finetuning small pretrained encoders (e.g., BERT and its variants) as well as small language models~\cite{phi2, gemma} has proven effective~\cite{sun2019fine} and cost-efficient~\cite{tsai2019small}. However, end-to-end (E2E) finetuning loses pretraining knowledge and is subject to overfitting risks and instability~\cite{mosbach2020stability}, especially with smaller finetuning datasets. The class of \textit{sparse finetuning methods} is designed to modify only a focused subset of the model parameters~\cite{neft, lester2021power, li2021prefix} for a new domain or task, thus mitigating the above risks. However, compared to E2E finetuning, they show performance limitations when the domain gap is large~\cite{liu2022improved}. In this paper, we answer the following question -- Can we combine the \emph{flexiblity and accuracy} of end-to-end finetuning with the \emph{stability and efficiency} of sparse finetuning for accurate and efficient semantic classification?





We identify token-driven parameter selection as the bridge to achieve task adaptation while retaining pretraining knowledge and the stability advantages of sparse finetuning. Our key insight is the following. By introducing task-specific phrases, token constructs, and subsequences to the model vocabulary, we can effectively estimate the sensitivity of each model parameter on the task-specific finetuning data. We then selectively finetune sensitive parameters for task adaptation while leaving most of the pretrained weights unchanged, thus reducing the risks of overfitting and providing greater stability compared to E2E finetuning. Compared to task-agnostic sparse finetuning methods (LoRA and its variants~\cite{zhang2023adalora, valipour2022dylora}, heurstic parameter selection~\cite{neft}, or prefix-tuning~\cite{li2021prefix}), our approach enables focused adaptation to the classification task without adding any new parameters to the pretrained model. Past work supports our insight - domain-specific subwords reduce the need to pretrain from scratch on new domains~\cite{aws, zouhar2023tokenization, multigrain}.

Thus, in summary, we identify the most sensitive subset of model parameters that can be finetuned to seamlessly integrate task-specific supervised classification labels with the pretraining weights of the model. This includes representations for the newly introduced task-specific token constructs in \cref{fig:intro1}, as well as the most sensitive layer parameters and weights to adapt to the task. Our work thus addresses the limitations of both E2E finetuning and task-agnostic sparse finetuning approaches with a two-pronged solution: sparse finetuning synergized with task-specific tokenization for efficient adaptation of pretrained models. We make the following contributions in this work:

\begin{itemize}
\item We develop a novel sparse finetuning approach for specialized semantic classification tasks by leveraging task-specific token constructs (individual tokens, token sequences - both contiguous and non-contiguous) for parameter selection. In contrast to previous parameter-efficient finetuning approaches which do not customize per-task, we introduce task-specific tokenization and parameter selection to enable customized finetuning per classification task.

\item We extensively evaluate our proposed task-adaptation approach against three broad model adaptation approaches: end-to-end finetuning, low-rank adaptation, and prefix tuning. We consistently outperform these approaches on five diverse semantic classification tasks.
\end{itemize}


% In recent years, the landscape of artificial intelligence and natural language processing has been significantly transformed by the advent of pre-trained language models (LMs) such as BERT (Bidirectional Encoder Representations from Transformers). These models have demonstrated unparalleled capabilities in understanding and generating human language, propelling a wide array of applications across various domains. At the heart of these advances is the ability of such models to capture the intricacies of language through comprehensive pre-training on diverse datasets, followed by fine-tuning on specific domain data to tailor their capabilities to specialized verticals. This process of fine-tuning pre-trained language models on domain-specific data presents a promising avenue for deploying cutting-edge AI capabilities that are acutely sensitive to the unique language properties and challenges of different fields. However, the efficacy of fine-tuning is intricately tied to the strategies employed during this phase, particularly concerning the input structure, which is fundamentally influenced by the tokenization strategy, tokenizer vocabulary, and token structure in the input samples.

% Tokenization, the process of converting input text into a sequence of tokens or symbols that a model can understand, plays a pivotal role in the performance of fine-tuned language models. The choice of tokenization strategy can dramatically affect a model's ability to interpret and generate domain-specific language accurately. In light of this, our work delves into the critical aspects of tokenization that must be considered when fine-tuning language models for domain-specific tasks. Specifically, we identify three key criteria that significantly influence the success of these endeavors: the availability of domain-specific tokens, the granularity of tokenization, and the structure of input tokens.

% This involves enriching the model's vocabulary with tokens, sequences, and other constructs that capture the specialized language of the field, thereby enhancing its understanding and generation capabilities. The structure and sequencing of input tokens influence its ability to learn from small volumes of domain-specific annotated data. The arrangement and grouping of tokens enable a more efficient encoding of the relationships between different pieces of information in the text, thereby improving training data efficiency.

 

% Secondly, choosing the right token granularity is crucial for balancing the model's computational efficiency and its ability to capture nuanced meanings. Finer granularity, where tokens represent smaller units of language, can lead to a more detailed understanding of the text but may increase the model's complexity and inference costs. Conversely, coarser granularity reduces the model's computational burden but may compromise its ability to grasp subtle distinctions in meaning.

% Thirdly, 

% Our investigation reveals that each of these tokenization criteria has a directional impact on the fine-tuned model's domain performance, its ability to generalize to new samples or tasks, and the associated inference costs. Furthermore, we demonstrate that these considerations come with inherent trade-offs. For instance, specializing tokenizers to enhance domain-specific performance can inadvertently lead to models that are more brittle, potentially compromising their robustness and generalizability across broader contexts.

% Therefore, finding the optimal balance among these trade-offs is essential for maximizing the benefits of fine-tuning while maintaining the overall robustness and generalizability of the models. Our contributions in this regard include a comprehensive analysis of the effects of different tokenization strategies on model performance, insights into how to navigate the trade-offs associated with these strategies, and guidelines for selecting the most effective tokenization criteria for domain-specific fine-tuning. Through this work, we aim to provide a foundation for further research and development in the field, enabling more effective and efficient use of fine-tuned language models across a variety of specialized verticals.




==> sections/old/methodology.tex <==
\section{Prototype-then-edit Model}
\label{sec:ne_model}

\citet{guu2018generating} introduce a novel unconditional generative model that samples a ``prototype'' sentence from the training corpus and edits it using a randomly sampled edit vector. The authors find that within the Yelp restaurant review corpus, 70\% of the test set is within a Jaccard distance of 0.5 of a training set sentence, implying that a neural editor with smooth and consistent edits should capture the test set. There are two significant constraints for the edit model:
\begin{itemize}
    \item \textbf{Semantic Smoothness}: Edits should change the semantics of text by a small amount and, when stacked together, create a larger change.
    \item \textbf{Consistent Edit Behavior}: The edit vector, $z$, should control the change in a sentence such that when applied to different sentences, the edits are semantically analogous.
\end{itemize}

% We provide details into how \cite{guu2018generating} define their model. 
The likelihood of a sentence is formulated as $p(x) = \sum_{x' \in \mathcal{X}} p(x | x') p(x')$ where $x'$ is prototype sentence and $x$ is the generated sentence. We define $p(x | x') = \mathbb{E}_{z \sim p(z)} [p_{edit}(x | x', z)]$ where $p_{edit}(x | x', z)$ is our neural editor. A sum over all prototypes $x'$ is expensive so we only sum over the $x'$ that are lexically similar to $x$ - a lexical similarity neighborhood, $\mathcal{N}(x)$. 


% $$p(x) = \sum_{x' \in \mathcal{X}} p(x | x') p(x')$$

% where $x'$ is prototype sentence, $x$ is the generated sentence, and  $p(x | x') = \mathbb{E}_{z \sim p(z)} [p_{edit}(x | x', z)]$. However, since this requires a sum over all prototypes $x'$, the authors only sum over the $x'$ that are lexically similar to $x$. They create a lexical similarity neighborhood:

% $$\mathcal{N}(x) = \{x' \in \mathcal{X} : d_J(x, x') < 0.5\}$$

% where $d_J$ is the Jaccard distance. The  model is trained by maximizing the marginal likelihood, $p(x)$, with gradient ascent. However, $p(x|x')$ has no closed-form solution, which is solved by lower bounding the expectation with the evidence lower bound (ELBO) \cite{kingma2013auto} 

% Ultimately, 
The model features three main components: a neural editor $p_{edit}(x | x', z)$, an inverse neural editor $q(z | x', x)$, and an edit prior $p(z)$. Note that the neural editor and inverse neural editor combine to form a VAE. The neural editor is implemented as a sequence-to-sequence model with attention, where given $x'$ as input and $z$, which is concatenated to the input of the decoder at each step, it ultimately generates $x$. The edit prior $z = z_{norm} \cdot z_{dir}$ where $z_{norm}$, the strength of the edit, is drawn from $\mathcal{U}(0,10)$ and $z_{dir}$, the direction of the edit, is sampled from a uniform distribution on the unit sphere. The inverse neural editor is given the edit pair $(x, x')$ and must infer the edit vector $z$. The difference between $x$ and $x'$ is represented as

$$f(x, x') = \sum_{w \in I} \Phi(w) \oplus \sum_{w \in D} \Phi(w)$$

where $I = x \setminus x'$ (\ie the set of words added to $x'$), $D = x \setminus x'$ (\ie the set of words deleted from $x'$), and $\Phi(w)$ is the GloVe \cite{pennington2014glove} vector for $w$. The inverse neural editor outputs a perturbed version of $f(x, x')$ as the edit vector, as follows:

$$q(z_{dir} | x', x) = \text{vMF}(f_{dir}, \kappa)$$
$$q(z_{norm} | x', x) = \mathcal{U}(f_{norm}, f_{norm} + \epsilon)$$

where $f_{norm} = \min(\|f\|, 10 - \epsilon)$ and $f_{dir} = \frac{f}{f_{norm}}$. Let $\text{vMF}(\mu, \kappa)$ be a von-Mises Fisher distribution where $\mu$ is the mean vector, and $\kappa$ is the concentration parameter.\footnote{$\kappa$ controls the rate of decay as the log-likelihood of a point decays linearly with the cosine similarity to $\mu$ in vMF distributions}

\section{Controllable Edit Vectors}
\label{sec:ne_edits}

% In order to introduce a control mechanism for our target features, we alter two aspects of the prototype-then-edit model: neighborhood creation and edit vector perturbation.
To exhibit control over our target attributes, we alter the prototype-then-edit model in two ways: neighborhood creation and edit vector perturbation. The former constrains the edit prior to edit vectors that demonstrate the desired change in attribute, within some tolerance $\epsilon$. The latter encourages a perturbation to the edit vector in the desired direction to compensate for $\epsilon$.

\textbf{Constrained Neighborhood Creation}: The model's behavior is heavily constrained by the lexical similarity condition in the creation of the neighborhood. By creating an additional constraint on the target attribute, we can ensure that edit vectors drawn from $p(z)$ correspond to a specified change in that attribute. More formally, we define the neighborhood as

\begin{align*}
    \mathcal{N}_{\Delta}(x) &= \{x' \in \mathcal{X} : d_J(x, x') < 0.5, \\
                            &  \hspace{0.3in} |(s(x) - s(x')) - \Delta| \leq \epsilon \}
\end{align*}

where $s(\cdot)$ computes the target attribute given text, $\delta$ is a desired change in the target attribute, and $\epsilon$ is the tolerance.
% Note that direction is enforced with $(s(x) - s(x'))$.

\textbf{Controlled Edit Vector Peturbation}: We hypothesize that by altering the magnitude of $z_{norm}$ and the direction $z_{dir}$, we can control the strength and behavior of the edit vector. Expressly, we can condition the formulation of the inverse neural editor on the target attribute by defining $q(z_{norm} | x', x) = \mathcal{N}(\Delta, 1) \cdot \mathcal{U}(f_{norm}, f_{norm} + \epsilon)$, where $\mathcal{N}$ is the normal distribution, $\mathcal{U}$ is the uniform distribution, and $\Delta$ is the desired change in the target attribute.


==> sections/results_fig.tex <==
\section{Results}
\label{sec:ne_results}

% \footnote{The variance across runs is generally negligible for each metric (\eg $0.005$ for BERTScore) and thus we omit it from tables, only reporting the averaged metric.} 

\begin{figure*}[]
  \centering
  \caption{Percent errors for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. We find that our approaches (\textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) show significantly more control over all control conditions across nearly all target deltas.}
  \includegraphics[width=\textwidth]{figs/delta_comps.pdf}
  \label{fig:errors}
  \vspace{-15px}
\end{figure*}

In this section, we evaluate \textsc{Cev-LM} on the strength of control (\Cref{subsec:control_eval}) as well as the relevance to the original text (\Cref{subsec:semantic_sim} and~\Cref{subsec:lexical_sim}). In \Cref{subsec:tolerance}, we discuss tuning the tolerance hyperparameter and in~\Cref{subsec:tolerance}, the effect of the data distribution on training. We provide qualitative results in~\Cref{subsec:qualitative}.

\subsection{Control Evaluation}
\label{subsec:control_eval}

We use the out-of-the-box edit-then-prototype (\textsc{Edit-then-Prototype}) model to provide a baseline $\Delta$ for all evaluations (except in~\Cref{fig:errors}, as the error would almost always be $100\%$). We run all baselines three times and report the average.

~\Cref{fig:errors} show the percent error of each approach across various target deltas, while~\Cref{fig:bleu_bert} shows the BERT and BLEU scores. We find that \textsc{Cev-LM} exhibits significantly greater control of $\Delta$ over the baseline approaches while preserving lexical and semantic similarity across all three attributes and all target deltas.

The baselines generally yield fluent but not controlled text. GPT-3 often generates texts with minimal change in attribute (\ie $\Delta = 0$), showing it cannot understand these nonstandard control conditions through few-shot learning. Conversely, prefix-tuning can replicate the attributes somewhat well but falls short due to neural hallucinations and poor-quality text. In low-resource scenarios (\ie high target deltas and fewer training samples), prefix-tuning led to significant over- or under-fitting; thus, we omit the results. In many cases, MuCoCO and SSD-LM perform poorly in terms of percent error but sometimes outperform or perform on par with our approaches. While we cannot fully explain this behavior, we hypothesize that the data distribution of $\Delta$ in $\mathcal{N}(x)$ plays a significant role. In some cases, we see strong results with both \textsc{Cev-LM} modifications, indicating that combining the modifications is beneficial with certain attributes and when $\epsilon$ is tuned. Specifically, volume consistently benefits from controlled edit vector perturbation, while speed and circuitousness show conflicting results. We find that circuitousness has much larger errors on average, likely due to the dependency on computing the shortest path.

% We plot these distributions in~\Cref{fig:feature_distr} and provide further reasoning in~\Cref{appendix:data_dist}.
\subsection{Semantic Similarity}
\label{subsec:semantic_sim}

In the first subfigure of~\Cref{fig:bleu_bert}, we report the BERT Scores of all approaches across various target deltas for each nonstandard control condition. We observe that \textsc{Cev-LM} consistently outperforms the other approaches while performing about on par with the edit-then-prototype baseline. This demonstrates that our approach preserves semantic similarity while significantly changing the speed, volume, or circuitousness of the text (also seen in~\Cref{tab:eval}). As the target delta increases, the BERT Score of our approach tends to decrease. We explain this phenomenon further in~\Cref{subsec:data_dist}.

% ================================================================================================
\begin{figure*}[]
  \centering
  \caption{BLEU and BERT (F1) scores for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.}
  \includegraphics[width=\textwidth]{figs/bert_comps.pdf}
  \includegraphics[width=\textwidth]{figs/bleu_comps.pdf}
  \label{fig:bleu_bert}
  \vspace{-15px}
\end{figure*}
% ================================================================================================

% \begin{figure*}[]
%   \centering
%   \caption{BERT Scores (F1) for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.}
%   \includegraphics[width=\textwidth]{figs/bert_comps.pdf}
%   \label{fig:bert}
%   \vspace{-15px}
% \end{figure*}

\subsection{Lexical Similarity}
\label{subsec:lexical_sim}

In the latter part of~\Cref{fig:bleu_bert}, we report the BLEU Scores of all approaches across various target deltas for each nonstandard control condition. We generally observe similar trends for our approaches in that BLEU score decreases as target delta increases, although to a greater scale. Since BLEU score measures lexical similarity, it is more sensitive to changes in wording, leading to a larger spread of scores. We also find that unlike before, \textsc{Cev-LM} does not clearly outperform the other approaches, which may imply that it presents semantically similar content while changing the wording. 

% \begin{figure*}[]
%   \centering
%   \caption{BLEU scores for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.}
%   \includegraphics[width=\textwidth]{figs/bleu_comps.pdf}
%   \label{fig:bleu}
%   \vspace{-15px}
% \end{figure*}

% While speed and volume perform nearly identically in~\Cref{tab:eval}, both with low errors, volume reacts much better to edit vector perturbation.

\subsection{Tolerance Tuning}
\label{subsec:tolerance}

We measure the impact of $\epsilon$ on training, testing $\epsilon = \{0.05, 0.1, 0.2\}$. When tolerance is too low, the approach overfits from the lack of training data, leading to smaller percent errors and poor similarity metrics. Including controlled perturbations to edit vectors improves similarity metrics at the cost of $\Delta$, indicating that the approach may help combat overfitting.  The effect of controlled edit vector perturbation is inconsistent across tolerance values and attributes, so we use $\epsilon = 0.1$ to provide an effective balance of control over a certain $\Delta$ and enough data for robust training. More details can be found in~\Cref{appendix:tolerance}.

% It is likely that the perturbation benefits from having $\Delta$-constrained pairs but we leave it to future work to investigate this behavior.

\subsection{Training Delta Distribution}
\label{subsec:data_dist}

We analyze the distribution of $\Delta$ in $\mathcal{N}(x)$ in~\Cref{fig:feature_distr}. The distribution is centered at 0 and denser at smaller magnitudes of $\Delta$, implying a lack of training data for larger shifts in the target attribute. This explains the general trend of increasing MAE and decreasing BLEU/BERT score as the target delta increases, seen in~\Cref{tab:eval}.

\begin{figure*}[]
  \centering
  \caption{Histogram of delta values (\ie $s(x) - s(x')$) within the Yelp Restaurant Review Corpus. The x-axis represents the difference in speed within the pairs of our created neighborhood, $\mathcal{N}(x)$, without any constraint on speed. The y-axis counts the number of pairs exhibiting the given delta in log-scale.}
  \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/speed.pdf}}
  \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/volume.pdf}}
  \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/circuitousness.pdf}}
  \label{fig:feature_distr}
\end{figure*}

In~\Cref{fig:samples_vs_error}, we record the performance against the number of training samples, finding that despite fewer samples, control through low-resource training is just as successful as through high-resource training. While circuitousness is the worst-performing attribute, likely due to the complexity of capturing the shortest path-based computation, it surprisingly does worst in a high-resource setting. It is possible that the change in attribute was too small to capture, even with a high number of samples. We see some success with decreasing the number of samples by a few orders of magnitude while preserving performance, across all attributes but leave extensive investigation to future work.

\begin{figure}[]
  \centering
  \caption{The number of samples used for training versus percent error. The attribute is denoted by the shape, target delta by the color, and the border indicates that perturbation was used. Despite access to significantly fewer samples, low-resource models exhibit similar amounts of control to high-resource models.}
  \scalebox{0.7}{
  \includegraphics[width=0.68\textwidth]{figs/samples_vs_error.pdf}
  }
  \label{fig:samples_vs_error}
\end{figure}

\subsection{Qualitative Results}
\label{subsec:qualitative}

\Cref{tab:ne_speed_example,tab:ne_volume_example,tab:ne_circuitousness_example} show the generations of the \textsc{Edit-then-Prototype} Baseline, GPT-3, SSD-LM, and each of our methods (\ie \textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) with $\epsilon=0.1$ when given a target delta of $0.5$ for speed, volume, and circuitousness, respectively. 
In~\Cref{tab:ne_speed_example}, we observe that our approaches generations tend to convey the same information in a shorter span, indicating an increase in speed. GPT-3 is generally not consistent, and SSD-LM tends to stray off-topic. In~\Cref{tab:ne_volume_example}, we can see that our approach tends to add information/verbosity, indicating an increase in volume. Here, GPT-3 shows little to no change in generation, and again, SSD-LM tends to stray off-topic, hallucinating information. Lastly, in~\Cref{tab:ne_circuitousness_example}, our approach leads to more indirect descriptions. While the text is more verbose, like volume, it repeats information/words, a key facet of circuitousness. GPT-3 hardly changes the input, and SSD-LM hallucinates some information. 

In addition to qualitative observations comparing variations of our approach, ~\Cref{tab:eval} in~\Cref{appendix:perturb} shows the results of training without and with controlled edit vector perturbation, respectively, in comparison to a baseline edit-then-prototype model to show that our approach significantly changes the behavior of the edit-then-prototype model. 

% For both sequences, the generations of our modified models are much shorter while preserving content, indicating higher speed. The baseline for both prompts made minimal edits to the input sentences (\eg ``excellent'' to ``amazing''), resulting in close to no change in speed but an extremely high similarity. GPT-3 and SSD-LM both struggled to change the speed of the text and significantly strayed from the original text, sometimes changing the meaning. 

 

  \begin{table}[htb]
  \small
  \centering
  \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{speed}$ with a target delta of $0.5$. We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  \label{tab:ne_speed_example} 
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
   \toprule[1.5pt]
  \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Speed}}\\
  \midrule[0.75pt]
  \textsc{Example 1:}\\
  \textbf{Original}: He went above and beyond in providing us excellent customer service and was extremely courteous friendly and kind.  \\
  \textbf{\textsc{Edit-then-Prototype}}: He went above and beyond in providing us with amazing customer service and was extremely courteous friendly and kind.  \\
  \textbf{GPT-3}: He was a great customer service provider. He was friendly and kind, \\
  \textbf{SSD-LM}: I was pleased that this was in line with our expectations. Suggesting the right\\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Always amazing customer service and very knowlegable staff. \\
  \textbf{\textsc{Cev-LM}}: He was knowledgable, courteous, and went provided excellent customer service.\\
  \addlinespace[0.5em]
  \textsc{Example 2:}\\
  \textbf{Original}: The staff is very professional and friendly \& environment is clean.  \\
  \textbf{\textsc{Edit-then-Prototype}}: The staff is very professional and likable \& the environment is clean. \\
  \textbf{GPT-3}: The staff was very professional, but not too friendly. The environment was clean, \\
  \textbf{SSD-LM}: This is a great experience! Reviews the best experience in the world. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The friendly staff is very professional \& environment is clean. \\
  \textbf{\textsc{Cev-LM}}: Friendly staff and clean environment.\\
  \bottomrule[1.5pt]\\
  \end{tabularx}
  \vspace{-10px}
  \end{table}



  \begin{table}[htb]
  \small
  \centering
  \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{volume}$ with a target delta of $0.5$.  We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  \label{tab:ne_volume_example} 
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
   \toprule[1.5pt]
  \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Volume}}\\
  \midrule[0.75pt]
  \textsc{Example 1:}\\
  \textbf{Original}: Prices were very reasonable for the quality and quantity served.  \\
  \textbf{\textsc{Edit-then-Prototype}}: Prices were very reasonable for the quality and quantity of food there. \\
  \textbf{GPT-3}: The food was good, but the prices were a bit high for what \\
  \textbf{SSD-LM}: The manager seemed very pleased with the quantity and the good service. The manager was impressed by the price and quality. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The prices were quite reasonable for the quality and quantity of food that was presented. \\
  \textbf{\textsc{Cev-LM}}: And prices were surprisingly reasonable for the quality and quantity of food that was presented. \\
  \addlinespace[0.5em]
  \textsc{Example 2:}\\
  \textbf{Original}: I like this place--definitely going back. \\
  \textbf{\textsc{Edit-then-Prototype}}: I like going to this place for lunch. \\
  \textbf{GPT-3}: I really like this place. I'm definitely going back. \\
  \textbf{SSD-LM}: The service was quite good. The food was available and delicious for two hours. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Overall,everything was great and I'll be coming again next time. \\
  \textbf{\textsc{Cev-LM}}: Overall,had a great time and I'll definitely be back. \\
  \bottomrule[1.5pt]\\
  \end{tabularx}
  \vspace{-10px}
  \end{table}



  \begin{table}[htb]
  \small
  \centering
  \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{circuitousness}$ with a target delta of $0.5$.  We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  \label{tab:ne_circuitousness_example} 
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
   \toprule[1.5pt]
  \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Circuitousness}}\\
  \midrule[0.75pt]
  \textsc{Example 1:}\\
  \textbf{Original}: I've only tried their Thai food,so far,and it is very good. \\
  \textbf{\textsc{Edit-then-Prototype}}: I've only tried their Thai food,so far,and it is very good. \\
  \textbf{GPT-3}: I've only tried their Thai food, so far, and it was really \\
  \textbf{SSD-LM}: They are very good in preparing food. However, if the food is really not good, then the chicken you can eat. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
  \textbf{\textsc{Cev-LM}}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
  \addlinespace[0.5em]
  \textsc{Example 2:}\\
  \textbf{Original}: I'd give the decor 4 stars and the food 3 stars. \\
  \textbf{\textsc{Edit-then-Prototype}}: I'd give the service 2 stars and the food 3 stars. \\
  \textbf{GPT-3}: I'd give the decor 3 stars and the food 4 stars. \\
  \textbf{SSD-LM}: The food was not well-priced and expensive, but very well-made, and I was very pleased with it. \\
  \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: 3 stars for the food and 2 stars for the prices equals 2.5 stars for me. \\
  \textbf{\textsc{Cev-LM}}: I'd give 4 stars for the food and 3 stars for the service,3 stars for the decor. \\
  \bottomrule[1.5pt]\\
  \end{tabularx}
  \vspace{-10px}
  \end{table}
  
% GPT3
% MuCoCo, Target Delta: 0.5, Delta: -2.86743, BERT: 72.425, BLEU: 0.0312
% SSD-LM, Target Delta: 0.5, Delta: -0.31998, BERT: 84.422, BLEU: 0.0581

==> sections/results_tab.tex <==
\section{Results}
\label{sec:ne_results}



% PERCENT ERROR COMPUTATION SCRIPT
% s = s.replace("&", "").replace("\textbf{", "").replace("}", "").strip()
% while '  ' in s:
%     s = s.replace('  ', ' ')
    
% l = s.split()
% r = [0.125, 0.5, 2.0, 4.0, 0.125, 0.5, 2.0, 0.125, 0.5, 1.0]

% p = 0
% c = 0
% for x, y in zip(l, r):
%     if x == "-":
%         c += 1
%         continue
%     p += abs((float(x) - y)/y)
    
% print(p / (len(l) - c))

In this section, we evaluate \textsc{ADAPT} across all tasks and datasets on the two primary metrics - Efficiency (\Cref{subsec:efficiency}) and Overall Accuracy (\Cref{subsec:accuracy}). We then proceed to an ablation analysis in \Cref{subsec:ablation} to study the impact of each aspect - overall perplexity, surprise factor, and input structure. We also provide a tradeoff analysis for the model robustness against the granularity of the chosen tokens in \Cref{subsec:robustness}.

\subsection{Efficiency Results}
\label{subsec:efficiency}

\subsection{Overall Accuracy Results}
\label{subsec:accuracy}

\subsection{Ablation Analysis}
\label{subsec:ablation}

\subsection{Robustness and Granularity Analysis}
\label{subsec:robustness}

% \subsection{Control Evaluation}
% \label{subsec:control_eval}

% \Cref{tab:errors} show the achieved delta of each approach across various target deltas along with the average percent error, while~\Cref{tab:bleu_bert} shows the BERT and BLEU scores. We run all baselines three times and report the average. We find that \textsc{Cev-LM} exhibits significantly greater control of $\Delta$ over the baselines while preserving lexical and semantic similarity across all three attributes and all target deltas.

% The baselines generally yield fluent but not controlled text. GPT-3 often generates texts with minimal change in attribute (\ie $\Delta = 0$), showing it cannot understand these nonstandard control conditions through few-shot learning. Conversely, prefix-tuning can replicate the attributes somewhat well but falls short due to neural hallucinations and poor-quality text. In low-resource scenarios (\ie high target deltas and fewer training samples), prefix-tuning led to significant over- or under-fitting; thus, we omit the results. In many cases, MuCoCO and SSD-LM perform poorly in terms of percent error but sometimes outperform or perform on par with our approaches. While we cannot fully explain this behavior, we hypothesize that the data distribution of $\Delta$ in $\mathcal{N}(x)$ plays a significant role. In some cases, we see strong results with both \textsc{Cev-LM} modifications, indicating that combining the modifications is beneficial with certain attributes and when $\epsilon$ is tuned. Specifically, volume consistently benefits from controlled edit vector perturbation, while speed and circuitousness show conflicting results. We find that circuitousness has much larger errors on average, likely due to the dependency on computing the shortest path.

% We also evaluate on more commonly studied control attributes, formality and toxicity, and present the results in~\Cref{tab:other_attr_error}. Due to its definition, it is likely that \textsc{Cev-LM} is more suited to handle attributes defined with word embeddings. This seems to be reflected in the higher overall percent error, but \textsc{Cev-LM} still produces more controlled generations on both attributes than all other baselines, indicating the robustness of our approach. 

% \input{sections/tables/delta_tab_other_attr}

% \subsection{Semantic Similarity}
% \label{subsec:semantic_sim}

% \input{sections/tables/sim_tab}

% In the former part of~\Cref{tab:bleu_bert}, we report the BERT Scores of all approaches across various target deltas for each nonstandard control condition. We observe that \textsc{Cev-LM} consistently outperforms the other approaches while performing about on par with the edit-then-prototype baseline. This demonstrates that our approach preserves semantic similarity while significantly changing the speed, volume, or circuitousness of the text (also seen in~\Cref{tab:eval}). As the target delta increases, the BERT Score of our approach tends to decrease. We explain this phenomenon further in~\Cref{subsec:data_dist}. We include the scores for formality and toxicity in~\Cref{tab:other_bleu_bert}.

% \subsection{Lexical Similarity}
% \label{subsec:lexical_sim}

% In the latter part of~\Cref{tab:bleu_bert}, we report the BLEU Scores of all approaches across various target deltas for each nonstandard control condition. We generally observe similar trends for our approaches in that BLEU score decreases as target delta increases, although to a greater scale. Since BLEU score measures lexical similarity, it is more sensitive to changes in wording, leading to a larger spread of scores. We also find that unlike before, \textsc{Cev-LM} does not clearly outperform the other approaches, which may imply that it presents semantically similar content while changing the wording. We include the scores for formality and toxicity in~\Cref{tab:other_bleu_bert}.

% \subsection{Tolerance Tuning}
% \label{subsec:tolerance}

% We measure the impact of $\epsilon$ on $\Delta$ in~\Cref{tab:eval-tol} (see~\Cref{appendix:tolerance}), testing $\epsilon = \{0.05, 0.1, 0.2\}$. When tolerance is too low, the approach overfits from the lack of training data, leading to smaller percent errors and poor similarity metrics. Including controlled perturbations to edit vectors improves similarity metrics at the cost of $\Delta$, indicating that the approach may help combat overfitting.  The effect of controlled edit vector perturbation is inconsistent across tolerance values and attributes, so we use $\epsilon = 0.1$ to provide an effective balance of control over a certain $\Delta$ and enough data for robust training. More details can be found in~\Cref{appendix:tolerance}.

% % It is likely that the perturbation benefits from having $\Delta$-constrained pairs but we leave it to future work to investigate this behavior.

% \subsection{Training Delta Distribution}
% \label{subsec:data_dist}

% We analyze the distribution of $\Delta$ in $\mathcal{N}(x)$ in~\Cref{fig:feature_distr}. The distribution is centered at 0 and denser at smaller magnitudes of $\Delta$, implying a lack of training data for larger shifts in the target attribute. This explains the general trend of increasing MAE and decreasing BLEU/BERT score as the target delta increases, seen in~\Cref{tab:eval}.

% \begin{figure*}[!htbp]
%   \centering
%   \caption{Histogram of delta values (\ie $s(x) - s(x')$) within the Yelp Restaurant Review Corpus. The x-axis represents the difference in speed within the pairs of our created neighborhood, $\mathcal{N}(x)$, without any constraint on speed. The y-axis counts the number of pairs exhibiting the given delta in log-scale.}
%   \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/speed.pdf}}
%   \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/volume.pdf}}
%   \subfigure[]{\includegraphics[width=0.32\textwidth]{figs/circuitousness.pdf}}
%   \label{fig:feature_distr}
%   \vspace{-10pt}
% \end{figure*}

% In~\Cref{fig:samples_vs_error}, we record the performance against the number of training samples, finding that despite fewer samples, control through low-resource training is just as successful as through high-resource training. While circuitousness is the worst-performing attribute, likely due to the complexity of capturing the shortest path-based computation, it surprisingly does worst in a high-resource setting. It is possible that the change in attribute was too small to capture, even with a high number of samples. We see some success with decreasing the number of samples by a few orders of magnitude while preserving performance, across all attributes but leave extensive investigation to future work.

% \begin{figure}[!htbp]
%   \centering
%   \caption{The number of samples used for training versus percent error. The attribute is denoted by the shape, target delta by the color, and the border indicates that perturbation was used. Despite access to significantly fewer samples, low-resource models exhibit similar amounts of control to high-resource models.}
%   \scalebox{0.7}{
%   \includegraphics[width=0.68\textwidth]{figs/samples_vs_error_2.pdf}
%   }
%   \label{fig:samples_vs_error}
%   \vspace{-20pt}
% \end{figure}


% \subsection{Qualitative Results}
% \label{subsec:qualitative}

% \Cref{tab:ne_speed_example,tab:ne_volume_example,tab:ne_circuitousness_example} show the generations of the \textsc{Edit-then-Prototype} Baseline, GPT-3, SSD-LM, and each of our methods (\ie \textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) with $\epsilon=0.1$ when given a target delta of $0.5$ for speed, volume, and circuitousness, respectively. 
% In~\Cref{tab:ne_speed_example}, we observe that our approaches generations tend to convey the same information in a shorter span, indicating an increase in speed. GPT-3 is generally not consistent, and SSD-LM tends to stray off-topic. In~\Cref{tab:ne_volume_example}, we can see that our approach tends to add information/verbosity, indicating an increase in volume. Here, GPT-3 shows little to no change in generation, and again, SSD-LM tends to stray off-topic, hallucinating information. Lastly, in~\Cref{tab:ne_circuitousness_example}, our approach leads to more indirect descriptions. While the text is more verbose, like volume, it repeats information/words, a key facet of circuitousness. GPT-3 hardly changes the input, and SSD-LM hallucinates some information. 

% In addition to qualitative observations comparing variations of our approach,~\Cref{tab:eval} in~\Cref{appendix:perturb} shows the results of training without and with controlled edit vector perturbation, respectively, in comparison to a baseline edit-then-prototype model to show that our approach significantly changes the behavior of the edit-then-prototype model. We also include~\Cref{appendix:retrieval} to show qualitative examples of the retrieved prototypes.

% % For both sequences, the generations of our modified models are much shorter while preserving content, indicating higher speed. The baseline for both prompts made minimal edits to the input sentences (\eg ``excellent'' to ``amazing''), resulting in close to no change in speed but an extremely high similarity. GPT-3 and SSD-LM both struggled to change the speed of the text and significantly strayed from the original text, sometimes changing the meaning. 

% % \begin{table}[]
% %   \centering
% %   \small
% %   \caption{Strength of control on $\Delta$ for the trained models (ideally, $\Delta = 0.5$) for speed. The scores are averaged across three training runs with different seeds. We train a baseline edit-then-prototype model \cite{guu2018generating}, as well as \textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM} with different tolerances ($\epsilon$). We record both train and test BLEU to demonstrate overfitting with lower tolerances.}
% %   \label{tab:eval-tol-sm}
% %   \begin{tabularx}{0.9\linewidth}{@{}>{\raggedright\arraybackslash}Xc@{}}
% %    \toprule[1.5pt]
% %   \textsc{Model} & \textsc{Delta}  \\     
% %   \midrule[0.75pt]
% %   % \addlinespace[0.5em]
% % \textsc{Edit-then-Prototype}    & 0.0113  \\
% %   \midrule[0.75pt]
% % \textsc{Cev-LM ($\mathcal{N}$-only)}: $\epsilon$ = 0.05 & 0.4559  \\
% % \textsc{Cev-LM ($\mathcal{N}$-only)}: $\epsilon$ = 0.1  & 0.4558  \\
% % \textsc{Cev-LM ($\mathcal{N}$-only)}: $\epsilon$ = 0.2  & 0.4405  \\
% %   \midrule[0.75pt]
% % % Perturbation            & 0.4433 & 0.5513     & 0.4531    & 0.9346 \\
% % \textsc{Cev-LM}: $\epsilon$ = 0.05  & 0.4279  \\
% % \textsc{Cev-LM}: $\epsilon$ = 0.1   & 0.4455  \\
% % \textsc{Cev-LM}: $\epsilon$ = 0.2   & \textbf{0.4596}  \\
% %   \bottomrule[1.5pt]\\
% %   \end{tabularx}
% %   % \vspace{-10pt}
% %   \end{table}

%   \begin{table*}[!htbp]
%   \small
%   \centering
%   \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as the benchmarks and \textsc{Cev-LM} architectures for a change in $\textbf{speed}$ with a target delta of $0.5$. We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
%   \vspace{-5px}
%   \label{tab:ne_speed_example} 
%   \begin{tabularx}{\linewidth}{cl}
%    \toprule[1.5pt]
%   & \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Speed}}\\
%   \midrule[0.75pt]
%   % \textsc{Example 1:}\\
%   & \textbf{Original}: He went above and beyond in providing us excellent customer service and was extremely \\ & \hspace{36pt} courteous friendly and kind.  \\
%   & \textbf{\textsc{Edit-then-Prototype}}: He went above and beyond in providing us with amazing customer service and \\ & \hspace{36pt} was extremely courteous friendly and kind.  \\
%   \textsc{Example 1} & \textbf{GPT-3}: He was a great customer service provider. He was friendly and kind, \\
%   & \textbf{SSD-LM}: I was pleased that this was in line with our expectations. Suggesting the right\\
%   & \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Always amazing customer service and very knowlegable staff. \\
%   & \textbf{\textsc{Cev-LM}}: He was knowledgable, courteous, and went provided excellent customer service.\\
%   % \addlinespace[0.5em]
%   \midrule[0.75pt]
%   % \textsc{Example 2:}\\
%   & \textbf{Original}: The staff is very professional and friendly \& environment is clean.  \\
%   & \textbf{\textsc{Edit-then-Prototype}}: The staff is very professional and likable \& the environment is clean. \\
%   & \textbf{GPT-3}: The staff was very professional, but not too friendly. The environment was clean, \\
%   \textsc{Example 2} & \textbf{SSD-LM}: This is a great experience! Reviews the best experience in the world. \\
%   & \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The friendly staff is very professional \& environment is clean. \\
%   & \textbf{\textsc{Cev-LM}}: Friendly staff and clean environment.\\
%   \bottomrule[1.5pt]\\
%   \end{tabularx}
%   \vspace{-10px}
%   \end{table*}



%   \begin{table*}[!htbp]
%   \small
%   \vspace{-5pt}
%   \centering
%   \caption{Generations of the benchmarks and \textsc{Cev-LM} architectures for a change in $\textbf{volume}$ with a target delta of $0.5$. We use a tolerance $\epsilon = 0.1$ for all of our approaches. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
%   \vspace{-5px}
%   \label{tab:ne_volume_example} 
%   \begin{tabularx}{\linewidth}{cl}
%    \toprule[1.5pt]
%   & \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Volume}}\\
%   \midrule[0.75pt]
%   % \textsc{Example 1:}\\
%   & \textbf{Original}: Prices were very reasonable for the quality and quantity served.  \\
%   & \textbf{\textsc{Edit-then-Prototype}}: Prices were very reasonable for the quality and quantity of food there. \\
%   & \textbf{GPT-3}: The food was good, but the prices were a bit high for what \\
%   \textsc{Example 1} & \textbf{SSD-LM}: The manager seemed very pleased with the quantity and the good service. The manager was \\ & \hspace{37pt} impressed by the price and quality. \\
%   & \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The prices were quite reasonable for the quality and quantity of food that was presented. \\
%   & \textbf{\textsc{Cev-LM}}: And prices were surprisingly reasonable for the quality and quantity of food that was presented. \\
%   % \addlinespace[0.5em]
%   \midrule[0.75pt]
%   % \textsc{Example 2:}\\
%   & \textbf{Original}: I like this place--definitely going back. \\
%   & \textbf{\textsc{Edit-then-Prototype}}: I like going to this place for lunch. \\
%   & \textbf{GPT-3}: I really like this place. I'm definitely going back. \\
%   \textsc{Example 2} & \textbf{SSD-LM}: The service was quite good. The food was available and delicious for two hours. \\
%   & \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Overall,everything was great and I'll be coming again next time. \\
%   & \textbf{\textsc{Cev-LM}}: Overall,had a great time and I'll definitely be back. \\
%   \bottomrule[1.5pt]\\
%   \end{tabularx}
%   \vspace{-10px}
%   \end{table*}



%   \begin{table*}[!htbp]
%   \small
%   \vspace{-5pt}
%   \centering
%   \caption{Generations of the benchmarks and \textsc{Cev-LM} architectures for a change in $\textbf{circuitousness}$ with a target delta of $0.5$. We use a tolerance $\epsilon = 0.1$ for all of our approaches. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
%   \vspace{-5px}
%   \label{tab:ne_circuitousness_example} 
%   \begin{tabularx}{\linewidth}{cl}
%    \toprule[1.5pt]
%   & \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Circuitousness}}\\
%   \midrule[0.75pt]
%   % \textsc{Example 1:}\\
%   & \textbf{Original}: I've only tried their Thai food,so far,and it is very good. \\
%   & \textbf{\textsc{Edit-then-Prototype}}: I've only tried their Thai food,so far,and it is very good. \\
%   & \textbf{GPT-3}: I've only tried their Thai food, so far, and it was really \\
%   \textsc{Example 1} & \textbf{SSD-LM}: They are very good in preparing food. However, if the food is really not good, then the chicken \\ & \hspace{37pt} you can eat. \\
%   & \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
%   & \textbf{\textsc{Cev-LM}}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
%   % \addlinespace[0.5em]
%   \midrule[0.75pt]
%   % \textsc{Example 2:}\\
%   & \textbf{Original}: I'd give the decor 4 stars and the food 3 stars. \\
%   & \textbf{\textsc{Edit-then-Prototype}}: I'd give the service 2 stars and the food 3 stars. \\
%   & \textbf{GPT-3}: I'd give the decor 3 stars and the food 4 stars. \\
%   \textsc{Example 2} & \textbf{SSD-LM}: The food was not well-priced and expensive, but very well-made, and I was very pleased with it. \\
%   & \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: 3 stars for the food and 2 stars for the prices equals 2.5 stars for me. \\
%   & \textbf{\textsc{Cev-LM}}: I'd give 4 stars for the food and 3 stars for the service,3 stars for the decor. \\
%   \bottomrule[1.5pt]\\
%   \end{tabularx}
%   \vspace{-15px}
%   \end{table*} 


















  % \begin{table*}[htb]
  % \small
  % \centering
  % \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{speed}$ with a target delta of $0.5$. We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  % \vspace{-5px}
  % \label{tab:ne_speed_example} 
  % \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
  %  \toprule[1.5pt]
  % \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Speed}}\\
  % \midrule[0.75pt]
  % \textsc{Example 1:}\\
  % \textbf{Original}: He went above and beyond in providing us excellent customer service and was extremely courteous friendly and kind.  \\
  % \textbf{\textsc{Edit-then-Prototype}}: He went above and beyond in providing us with amazing customer service and was extremely courteous friendly and kind.  \\
  % \textbf{GPT-3}: He was a great customer service provider. He was friendly and kind, \\
  % \textbf{SSD-LM}: I was pleased that this was in line with our expectations. Suggesting the right\\
  % \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Always amazing customer service and very knowlegable staff. \\
  % \textbf{\textsc{Cev-LM}}: He was knowledgable, courteous, and went provided excellent customer service.\\
  % \addlinespace[0.5em]
  % \textsc{Example 2:}\\
  % \textbf{Original}: The staff is very professional and friendly \& environment is clean.  \\
  % \textbf{\textsc{Edit-then-Prototype}}: The staff is very professional and likable \& the environment is clean. \\
  % \textbf{GPT-3}: The staff was very professional, but not too friendly. The environment was clean, \\
  % \textbf{SSD-LM}: This is a great experience! Reviews the best experience in the world. \\
  % \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The friendly staff is very professional \& environment is clean. \\
  % \textbf{\textsc{Cev-LM}}: Friendly staff and clean environment.\\
  % \bottomrule[1.5pt]\\
  % \end{tabularx}
  % \vspace{-10px}
  % \end{table*}



  % \begin{table*}[htb]
  % \small
  % \centering
  % \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{volume}$ with a target delta of $0.5$.  We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  % \vspace{-5px}
  % \label{tab:ne_volume_example} 
  % \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
  %  \toprule[1.5pt]
  % \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Volume}}\\
  % \midrule[0.75pt]
  % \textsc{Example 1:}\\
  % \textbf{Original}: Prices were very reasonable for the quality and quantity served.  \\
  % \textbf{\textsc{Edit-then-Prototype}}: Prices were very reasonable for the quality and quantity of food there. \\
  % \textbf{GPT-3}: The food was good, but the prices were a bit high for what \\
  % \textbf{SSD-LM}: The manager seemed very pleased with the quantity and the good service. The manager was impressed by the price and quality. \\
  % \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: The prices were quite reasonable for the quality and quantity of food that was presented. \\
  % \textbf{\textsc{Cev-LM}}: And prices were surprisingly reasonable for the quality and quantity of food that was presented. \\
  % \addlinespace[0.5em]
  % \textsc{Example 2:}\\
  % \textbf{Original}: I like this place--definitely going back. \\
  % \textbf{\textsc{Edit-then-Prototype}}: I like going to this place for lunch. \\
  % \textbf{GPT-3}: I really like this place. I'm definitely going back. \\
  % \textbf{SSD-LM}: The service was quite good. The food was available and delicious for two hours. \\
  % \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: Overall,everything was great and I'll be coming again next time. \\
  % \textbf{\textsc{Cev-LM}}: Overall,had a great time and I'll definitely be back. \\
  % \bottomrule[1.5pt]\\
  % \end{tabularx}
  % \vspace{-10px}
  % \end{table*}



  % \begin{table*}[htb]
  % \small
  % \centering
  % \caption{Generations of the baseline \cite{guu2018generating} ($\textbf{\textsc{Edit-then-Prototype}}$) as well as multiple variants of the baseline for a change in $\textbf{circuitousness}$ with a target delta of $0.5$.  We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. The models are fed the input (\ie \textbf{Original}) and generate by applying an ``edit vector'' to the latent representation of the input sentence.}
  % \vspace{-5px}
  % \label{tab:ne_circuitousness_example} 
  % \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}X@{}}
  %  \toprule[1.5pt]
  % \textsc{Model} \& \textsc{Generated Text} - \textbf{\textsc{Circuitousness}}\\
  % \midrule[0.75pt]
  % \textsc{Example 1:}\\
  % \textbf{Original}: I've only tried their Thai food,so far,and it is very good. \\
  % \textbf{\textsc{Edit-then-Prototype}}: I've only tried their Thai food,so far,and it is very good. \\
  % \textbf{GPT-3}: I've only tried their Thai food, so far, and it was really \\
  % \textbf{SSD-LM}: They are very good in preparing food. However, if the food is really not good, then the chicken you can eat. \\
  % \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
  % \textbf{\textsc{Cev-LM}}: I've decided that their Thai food is really good...their Japanese food,not so much. \\
  % \addlinespace[0.5em]
  % \textsc{Example 2:}\\
  % \textbf{Original}: I'd give the decor 4 stars and the food 3 stars. \\
  % \textbf{\textsc{Edit-then-Prototype}}: I'd give the service 2 stars and the food 3 stars. \\
  % \textbf{GPT-3}: I'd give the decor 3 stars and the food 4 stars. \\
  % \textbf{SSD-LM}: The food was not well-priced and expensive, but very well-made, and I was very pleased with it. \\
  % \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)}: 3 stars for the food and 2 stars for the prices equals 2.5 stars for me. \\
  % \textbf{\textsc{Cev-LM}}: I'd give 4 stars for the food and 3 stars for the service,3 stars for the decor. \\
  % \bottomrule[1.5pt]\\
  % \end{tabularx}
  % \vspace{-10px}
  % \end{table*}
  
% GPT3
% MuCoCo, Target Delta: 0.5, Delta: -2.86743, BERT: 72.425, BLEU: 0.0312
% SSD-LM, Target Delta: 0.5, Delta: -0.31998, BERT: 84.422, BLEU: 0.0581

==> sections/tables/delta_tab.tex <==
% \newcommand*{\newfactor}{0.056}
% \begin{table*}[h]
% \centering
% \tiny
% \caption{Achieved delta for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. We find that our approaches (\textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) show significantly more control over all control conditions across nearly all target deltas.\vspace{-5pt}}
% %\footnotesize
% \noindent\setlength\tabcolsep{2.9pt}
% % \fontsize{9pt}{9pt}\selectfont
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}p{0.20\linewidth}@{\hspace{2pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{}} \\
% \toprule
% \multirow{}{}{\textbf{Metric}} & \multicolumn{4}{c}{\textbf{Speed}}  & \multicolumn{3}{c}{\textbf{Volume}} & \multicolumn{3}{c}{\textbf{Circuitousness}} \\
% \cmidrule{2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
% %\midrule
% \multirow{}{}{\textbf{Target Delta}} & \textbf{0.125} & \textbf{0.5} & \textbf{2.0} & \textbf{4.0} & \textbf{0.125} & \textbf{0.5}& \textbf{2.0} & \textbf{0.125} & \textbf{0.5}& \textbf{1.0}\\

% \midrule
% \multicolumn{11}{c}{\textsc{Benchmark Approaches}} \\
% \midrule[0pt]

% \textbf{GPT-3}~\cite{brown2020language}       & -0.091 & 0.023  & 0.200 & 0.294 & 0.019 & 0.150 & 1.769 & 0.011  & 0.009         & 0.021 \\
% \textbf{MuCoCO}~\cite{kumar2021controlled}   & 0.169 & 0.871 & 1.293 & 3.610 & 0.142 & 0.558 & 2.310 & 0.068  & 0.058         & 0.054 \\
% \textbf{SSD-LM}~\cite{han2022ssd}    & 0.412 & 0.335  & 1.094 & 1.059 & 0.369 & 0.283 & 0.671 & \textbf{0.075}  & 0.078         & 0.109  \\
% \textbf{Prefix Tuning}~\cite{li2021prefix}  & 0.197 & 0.245 & 1.562 & -       & 0.088 & 0.877 &  -      & -0.004 & 0.159         & -  \\

% \midrule[0pt]
% \multicolumn{11}{c}{\textsc{Our Approaches}} \\
% \midrule[0pt]

% \textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)} & 0.111 & \textbf{0.457} & \textbf{1.760} & \textbf{3.621} & 0.111 & 0.443 & 1.752  & \textbf{0.072}  & 0.423          & \textbf{0.790} \\
% \textbf{\textsc{Cev-LM}} & \textbf{0.118} & 0.450 & 1.755 & 3.547 & \textbf{0.114} & \textbf{0.451} & \textbf{1.863} & 0.064  & \textbf{0.431}         & 0.781 \\

% \bottomrule
% \end{tabular}}
% \vspace{-10pt}
% \label{tab:errors}
% \end{table*}
% \newcolumntype{K}[1]{>{\centering\arraybackslash}p{#1}}
\newcommand*{\newfactor}{0.056}
\begin{table*}[!htbp]
\centering
\tiny
\caption{Achieved delta for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. We find that our approaches (\textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) show significantly more control over all control conditions across nearly all target deltas.\vspace{-5pt}}
%\footnotesize
\noindent\setlength\tabcolsep{2.9pt}
% \fontsize{8pt}{7pt}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.20\linewidth}@{\hspace{2pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{}} \\
ccc@{\hspace{5pt}}ccc@{\hspace{5pt}}ccc@{\hspace{5pt}}ccc@{}} \\
\toprule
{\textbf{Metric}} & \multicolumn{4}{c}{\textbf{Speed}}  & \multicolumn{3}{c}{\textbf{Volume}} & \multicolumn{3}{c}{\textbf{Circuitousness}} & \multicolumn{1}{c}{\textbf{\% Err}}\\
\cmidrule{2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule{12-12}
%\midrule
 {\textbf{Target Delta}} & \textbf{0.125} & \textbf{0.5} & \textbf{2.0} & \textbf{4.0} & \textbf{0.125} & \textbf{0.5}& \textbf{2.0} & \textbf{0.125} & \textbf{0.5}& \textbf{1.0} & -\\

\midrule
\multicolumn{11}{c}{\textsc{Benchmark Approaches}} \\
\midrule[0pt]

\textbf{GPT-3}~\cite{brown2020language}       & -0.091 & 0.023  & 0.200 & 0.294 & 0.019 & 0.150 & 1.769 & 0.011  & 0.009         & 0.021 & 90.44 \\
\textbf{MuCoCO}~\cite{kumar2021controlled}   & 0.169 & 0.871 & 1.293 & 3.610 & 0.142 & 0.558 & 2.310 & 0.068  & 0.058         & 0.054 & 42.38 \\
\textbf{SSD-LM}~\cite{han2022ssd}    & 0.412 & 0.335  & 1.094 & 1.059 & 0.369 & 0.283 & 0.671 & \textbf{0.075}  & 0.078         & 0.109 & 90.00 \\
\textbf{Prefix Tuning}~\cite{li2021prefix}  & 0.197 & 0.245 & 1.562 & -       & 0.088 & 0.877 &  -      & -0.004 & 0.159         & -  & 58.12 \\

\midrule[0pt]
\multicolumn{11}{c}{\textsc{Our Approaches}} \\
\midrule[0pt]

\textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)} & 0.111 & \textbf{0.457} & \textbf{1.760} & \textbf{3.621} & 0.111 & 0.443 & 1.752  & \textbf{0.072}  & 0.423          & \textbf{0.790} & 15.51 \\
\textbf{\textsc{Cev-LM}} & \textbf{0.118} & 0.450 & 1.755 & 3.547 & \textbf{0.114} & \textbf{0.451} & \textbf{1.863} & 0.064  & \textbf{0.431}         & 0.781 & \textbf{14.91}\\

\bottomrule
\end{tabular}}
\vspace{-10pt}
\label{tab:errors}
\end{table*}

==> sections/tables/delta_tab_other_attr.tex <==

\begin{table*}[!htbp]
\centering
\tiny
\caption{Achieved delta for toxicity and formality across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}. We find that our approaches (\textsc{Cev-LM ($\mathcal{N}$-only)} and \textsc{Cev-LM}) show significantly more control over all control conditions across nearly all target deltas.\vspace{-5pt}}
%\footnotesize
\noindent\setlength\tabcolsep{2.9pt}
\fontsize{5pt}{6pt}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.20\linewidth}@{\hspace{2pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% % K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{}} \\
ccc@{\hspace{5pt}}ccc@{\hspace{5pt}}ccc@{}}
\toprule
{\textbf{Metric}} & \multicolumn{3}{c}{\textbf{Toxicity}}  & \multicolumn{3}{c}{\textbf{Formality}} & \multicolumn{1}{c}{\textbf{\% Err}}\\
\cmidrule{2-4} \cmidrule(lr){5-7} \cmidrule{8-8}
%\midrule
{\textbf{Target Delta}} & \textbf{0.1} & \textbf{0.5} & \textbf{0.9} & \textbf{0.1} & \textbf{0.5} & \textbf{0.9}& - \\

\midrule
% Metric        &       & Toxicity &       &       & Formality &       & \multicolumn{1}{c}{% Err} \\
% Target Delta  & 0.1   & 0.5      & 0.9   & 0.1   & 0.5    & 0.9   & \multicolumn{1}{c}{-}     \\ \hline
% GPT-3         & 0.017 & 0.083    & 0.360 & 0.279 & 0.309  & 0.370 & 83.74                     \\
% MuCoCO        & 0.014 & 0.041    & 0.063 & 0.234 & 0.148  & 0.155 & 92.99                     \\
% SSD-LM        & 0.011 & 0.218    & 0.342 & 0.008 & 0.376  & 0.650 & 58.66                     \\
% Prefix Tuning & 0.188 & 0.397    & 0.978 & 0.273 & 0.339  & 0.941 & 54.50                     \\ \hline
% CEV-LM        & 0.075 & 0.325    & 0.709 & 0.162 & 0.427  & 0.810 & 27.97                    
\textbf{GPT-3}~\cite{brown2020language}      & 0.017 & 0.083    & 0.360 & 0.279 & 0.309  & 0.370 & 83.74 \\
\textbf{MuCoCO}~\cite{kumar2021controlled}   & 0.014 & 0.041    & 0.063 & 0.234 & 0.148  & 0.155 & 92.99 \\
\textbf{SSD-LM}~\cite{han2022ssd}            & 0.011 & 0.218    & 0.342 & 0.008 & 0.376  & 0.650 & 58.66  \\
\textbf{Prefix Tuning}~\cite{li2021prefix}   & 0.188 & \textbf{0.397}    & 0.978 & 0.273 & 0.339  & \textbf{0.941} & 54.50 \\
\midrule[0pt]
\textbf{\textsc{Cev-LM} (Ours)}                     & \textbf{0.075} & 0.325    & \textbf{0.709} & \textbf{0.162} & \textbf{0.427}  & 0.810 & \textbf{27.97}\\

\bottomrule
\end{tabular}}
% \vspace{-10pt}
\label{tab:other_attr_error}
\end{table*}



==> sections/tables/sim_tab.tex <==
\begin{table*}[h]
\centering
\tiny
\caption{BLEU and BERT (F1) Scores for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.\vspace{-5pt}}
%\footnotesize
\noindent\setlength\tabcolsep{2.9pt}
% \fontsize{9pt}{9pt}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.20\linewidth}@{\hspace{2pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{}} \\
ccc@{\hspace{5pt}}ccc@{\hspace{5pt}}ccc@{\hspace{5pt}}ccc@{}}
\toprule
{\textbf{Metric}} & \multicolumn{4}{c}{\textbf{Speed}}  & \multicolumn{3}{c}{\textbf{Volume}} & \multicolumn{3}{c}{\textbf{Circuitousness}} \\
\cmidrule{2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
%\midrule
{\textbf{Target Delta}} & \textbf{0.125} & \textbf{0.5} & \textbf{2.0} & \textbf{4.0} & \textbf{0.125} & \textbf{0.5}& \textbf{2.0} & \textbf{0.125} & \textbf{0.5}& \textbf{1.0}\\

\midrule
\multicolumn{11}{c}{\textsc{\textbf{BERTScore} - Benchmark Approaches}} \\
\midrule[0pt]

\textbf{GPT-3}~\cite{brown2020language}       & 0.910 & 0.919 & 0.916 & 0.904 & 0.914 & 0.916 & 0.887 & 0.89 & 0.881 & 0.832 \\
\textbf{MuCoCO}~\cite{kumar2021controlled}   & 0.657 & 0.760 & 0.571 & 0.728 & 0.670 & 0.684 & 0.615 & 0.740 & 0.568 & 0.552 \\
\textbf{SSD-LM}~\cite{han2022ssd}    & 0.841 & 0.840 & 0.823 & 0.821 & 0.835 & 0.833 & 0.825 & 0.846 & 0.840 & 0.822  \\
\textbf{Prefix Tuning}~\cite{li2021prefix}  & 0.895 & 0.904 & 0.891 & - & 0.879 & 0.901 & - & 0.888 & 0.850 & - \\

\midrule[0pt]
\multicolumn{11}{c}{\textsc{\textbf{BERTScore} - Our Approaches}} \\
\midrule[0pt]

\textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)} & \textbf{0.935} & 0.934 & \textbf{0.929} & 0.919 & \textbf{0.938} & \textbf{0.932} & \textbf{0.925} & 0.927 & \textbf{0.911} & \textbf{0.909} \\
\textbf{\textsc{Cev-LM}} & \textbf{0.935} & \textbf{0.939} & \textbf{0.928} & \textbf{0.923} & 0.935 & \textbf{0.931} & 0.921 & \textbf{0.931} & \textbf{0.909} & 0.835 \\

\midrule
\multicolumn{11}{c}{\textsc{\textbf{BLEU} - Benchmark Approaches}} \\
\midrule[0pt]

\textbf{GPT-3}~\cite{brown2020language}       & 0.233 & 0.261 & \textbf{0.321} & 0.225 & 0.219 & \textbf{0.304} & 0.203 & 0.182 & 0.187 & 0.155 \\
\textbf{MuCoCO}~\cite{kumar2021controlled}   & 0.326 & \textbf{0.325} & 0.278 & 0.218 & 0.256 & 0.244 & 0.221 & 0.318 & 0.242 & 0.254 \\
\textbf{SSD-LM}~\cite{han2022ssd}    & 0.247 & 0.246 & 0.233 & \textbf{0.283} & 0.318 & 0.298 & 0.261 & \textbf{0.321} & \textbf{0.279} & \textbf{0.274}  \\
\textbf{Prefix Tuning}~\cite{li2021prefix}  & 0.231 & 0.217 & 0.230 & - & 0.224 & 0.255 & - & 0.268 & 0.246 & - \\

\midrule[0pt]
\multicolumn{11}{c}{\textsc{\textbf{BLEU} - Our Approaches}} \\
\midrule[0pt]

\textbf{\textsc{Cev-LM} ($\mathcal{N}$-only)} & \textbf{0.340} & \textbf{0.327} & 0.305 & 0.246 & \textbf{0.329} & 0.268 & \textbf{0.287} & 0.249 & 0.268 & 0.248 \\
\textbf{\textsc{Cev-LM}} & 0.326 & 0.313 & 0.295 & 0.273 & 0.304 & 0.265 & 0.252 & 0.290 & 0.276 & 0.162 \\

\bottomrule
\end{tabular}}
\label{tab:bleu_bert}
\vspace{10pt}
\end{table*}

==> sections/tables/sim_tab_other_attrs.tex <==
\begin{table*}[h]
\centering
\tiny
\caption{BLEU and BERT (F1) Scores for speed, volume, and circuitousness across all approaches for different target deltas. The scores are averaged across three training runs (inference runs for GPT-3). We use a tolerance $\epsilon = 0.1$ for all of our approaches, as it empirically provided the best results in~\Cref{subsec:tolerance}.\vspace{-5pt}}
%\footnotesize
\noindent\setlength\tabcolsep{2.9pt}
\fontsize{4pt}{4pt}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{0.20\linewidth}@{\hspace{2pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% % K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{\hspace{5pt}}
% K{\newfactor\linewidth}K{\newfactor\linewidth}K{\newfactor\linewidth}@{}} \\
ccc@{\hspace{5pt}}ccc@{\hspace{5pt}}ccc@{}}
\toprule
\textbf{Metric} & \multicolumn{3}{c}{\textbf{Toxicity}}  & \multicolumn{3}{c}{\textbf{Formality}}\\
\cmidrule{2-4} \cmidrule(lr){5-7}
%\midrule
{\textbf{Target Delta}} & \textbf{0.1} & \textbf{0.5} & \textbf{0.9} & \textbf{0.1} & \textbf{0.5} & \textbf{0.9} \\

\midrule
\multicolumn{7}{c}{\textsc{\textbf{BERTScore} - Benchmark Approaches}} \\
\midrule[0pt]

\textbf{GPT-3}~\cite{brown2020language}       & 0.857 & 0.869    & 0.866 & 0.851 & 0.851  & 0.862  \\
\textbf{MuCoCO}~\cite{kumar2021controlled}    & 0.763 & 0.771    & 0.774 & 0.763 & 0.759  & 0.760  \\
\textbf{SSD-LM}~\cite{han2022ssd}             & 0.769 & 0.767    & 0.769 & 0.763 & 0.760  & 0.747 \\
\textbf{Prefix Tuning}~\cite{li2021prefix}    & 0.833 & 0.827    & 0.823 & 0.843 & 0.836  & 0.834  \\ 

\midrule[0pt]
\multicolumn{7}{c}{\textsc{\textbf{BERTScore} - Our Approaches}} \\
\midrule[0pt]

\textbf{\textsc{Cev-LM}}                      & 0.848 & 0.827    & 0.837 & 0.842 & 0.842  & 0.845   \\

\midrule
\multicolumn{7}{c}{\textsc{\textbf{BLEU} - Benchmark Approaches}} \\
\midrule[0pt]

\textbf{GPT-3}~\cite{brown2020language}       & 0.231 & 0.250    & 0.291 & 0.219 & 0.273     & 0.269 \\
\textbf{MuCoCO}~\cite{kumar2021controlled}    & 0.305 & 0.268    & 0.293 & 0.257 & 0.276     & 0.219 \\
\textbf{SSD-LM}~\cite{han2022ssd}             & 0.294 & 0.343    & 0.346 & 0.314 & 0.325     & 0.326   \\
\textbf{Prefix Tuning}~\cite{li2021prefix}    & 0.246 & 0.269    & 0.275 & 0.231 & 0.217     & 0.194 \\

\midrule[0pt]
\multicolumn{7}{c}{\textsc{\textbf{BLEU} - Our Approaches}} \\
\midrule[0pt]

\textbf{\textsc{Cev-LM}}                      & 0.320 & 0.316    & 0.295 & 0.342 & 0.334     & 0.265 \\

\bottomrule
\end{tabular}}
\label{tab:other_bleu_bert}
% \vspace{-10pt}
\end{table*}


% \begin{table}[]
% \begin{tabular}{lcccccc}
% \hline
% BERTScore     &       & Toxicity &       &       & Formality &        \\
% Target Delta  & 0.1   & 0.5      & 0.9   & 0.1   & 0.5    & 0.9    \\ \hline
% GPT-3         & 85.65 & 86.89    & 86.58 & 85.08 & 85.12  & 86.20  \\
% MuCoCO        & 76.31 & 77.08    & 77.41 & 76.31 & 75.92  & 76.01  \\
% SSD-LM        & 76.86 & 76.66    & 76.87 & 76.27 & 75.96  & 0.7472 \\
% Prefix Tuning & 83.21 & 82.73    & 82.27 & 84.34 & 83.60  & 83.39  \\ \hline
% CEV-LM        & 84.81 & 82.70    & 83.69 & 84.18 & 84.19  & 84.47 
% \end{tabular}
% \end{table}

% \begin{table}[]
% \begin{tabular}{lcccccc}
% \hline
% BLEU          &       & Toxicity &       &       & Formality &       \\
% Target Delta  & 0.1   & 0.5      & 0.9   & 0.1   & 0.5       & 0.9   \\ \hline
% GPT-3         & 0.231 & 0.250    & 0.291 & 0.219 & 0.273     & 0.269 \\
% MuCoCO        & 0.305 & 0.268    & 0.293 & 0.257 & 0.276     & 0.219 \\
% SSD-LM        & 0.294 & 0.343    & 0.346 & 0.314 & 0.325     & 0.326 \\
% Prefix Tuning & 0.246 & 0.269    & 0.275 & 0.231 & 0.217     & 0.194 \\ \hline
% CEV-LM        & 0.320 & 0.316    & 0.295 & 0.342 & 0.334     & 0.265
% \end{tabular}
% \end{table}
